Assessing Post Deletion in Sina Weibo: Multi-modal Classification of Hot Topics

Widespread Chinese social media applications such as Weibo are widely known for monitoring and deleting posts to conform to Chinese government requirements. In this paper, we focus on analyzing a dataset of censored and uncensored posts in Weibo. Despite previous work that only considers text content of posts, we take a multi-modal approach that takes into account both text and image content. We categorize this dataset into 14 categories that have the potential to be censored on Weibo, and seek to quantify censorship by topic. Specifically, we investigate how different factors interact to affect censorship. We also investigate how consistently and how quickly different topics are censored. To this end, we have assembled an image dataset with 18,966 images, as well as a text dataset with 994 posts from 14 categories. We then utilized deep learning, CNN localization, and NLP techniques to analyze the target dataset and extract categories, for further analysis to better understand censorship mechanisms in Weibo. We found that sentiment is the only indicator of censorship that is consistent across the variety of topics we identified. Our finding matches with recently leaked logs from Sina Weibo. We also discovered that most categories like those related to anti-government actions (e.g. protest) or categories related to politicians (e.g. Xi Jinping) are often censored, whereas some categories such as crisis-related categories (e.g. rainstorm) are less frequently censored. We also found that censored posts across all categories are deleted in three hours on average.

==> discussion.tex <==
\section{Discussion}
%In this section, we discuss other aspects of Weibo's censorship. We first discuss long-term image censorship behavior in Weibo.

In this section, we discuss potential reasons for the results and address some potential concerns. We also provide the caveats about our study.

\subsection{Topics vs.\@ censorship}

\todo{Jed: could you please revise this section?}
One of our main results is that there is a high variance across topics in terms of the consistency with which posts in that topic are censored, as well as how quickly posts get censored.  There are several possible explanations for this, that are each interesting.  One possibility is that some topics are more sensitive than others.  For example, posts related to a protest event may be simply more objectionable from the censors' point of view than other topics.  Another possible explanation for the variance is that images can be sensitive or not depending on the sentiment of the text accompanying the image.  For example, a post with a picture of Mao may be accompanied by text either in support of or against Mao, but a post with a picture of making an X is always in opposition to China's policy towards Hong Kong.  
%We leave conclusively identifying the reasons for this variance in each case for future work, where we plan to take a multimodal approach (i.e., look at both images and text) and perform sentiment analysis. 
%\mct{Is it possible that our classifier might be missing the uncensored X makers for some reason?  Is it possible that some of our topics should be split into a sub-topics?}

\subsection{Long-term behavior}
It is possible that the behavior of the censors changes over a long period of time regarding some categories.
Thus, to investigate the long-term behavior of censors, we utilized the WeiboScope dataset because it was collected over a period of four years (from 2015 through 2018). Furthermore, this analysis helps us to address some potential concerns about our results. Regarding the censorship rates that we computed for each category, one might wonder whether time modulation might affect our results.
\mct{Can you define \emph{time modulation}?  I think you just mean changes over time or do mean something more precise.  Normally, I see ``modulation'' used in reference to a communication channel implying a highly controlled form of change over time.}
For example, Winnie the Pooh images may be 100\% censored currently now that they have became a meme referring to Xi Jinping's physical resemblance to Winnie the Pooh, but, in the past, they may have 0\% censored.
The net result will be an appearance in our dataset of some intermediate rate of censoring depending upon the how often Winnie the Pooh images appeared before and after becoming a censored.
In general, at some points in the past, the censors might have decided to start filtering some categories, and posts posted before that time might affect our results, or they might have censored some categories only for a short period of time.

Thus, to discover the long-term behavior with respect to each category and address the above-mentioned concerns, we compared the creation time of censored posts with that of uncensored posts in the same category. Figure~\ref{fig:time-weiboscope} depicts the creation time distribution of posts for the categories in WeiboScope dataset. The interesting points are summarized here:
%
%Regarding the censorship rates that we computed for each category, one might wonder that time modulation might affect our results, e.g. Winnie the Pooh images may be 100\% censored but 20\% of the images were posted before it became a meme that referred to Xi Jinping. In general, at some points in the past, the censors might have decided to start filtering some categories and images posted before that time might affect our results, or they might have censored some categories only for a short period of time. At the same time, since WeiboScope data is collected over almost four years, this dataset allows us to investigate these concerns. 
%
\begin{itemize}
    \item There is no point in time that shows the censors have started censoring a category from that point which means that the earliest censored post for each category is always at almost start of the dataset, and censored and uncensored posts in all categories have overlapping creation time. Thus it is safe to say that time modulation has not affected our results in a significant way, only in specific cases.
    \mct{Why?  That some are only censored in 2015 seems to suggest that time modulation could be happening at some low frequency.}
    \item Some categories, such as injury/dead, Bo Xilai, and prurient/nudity, are censored only in 2015. Therefore, it seems like these categories are less scrutinized after 2015, but this needs further investigation. 
    %Moreover, it seems like the censored images in the rainstorm category might be related to a major rainstorm in south China in 2015~\cite{rainstorm2015}.
\end{itemize}

\begin{figure}[!ht]
      \includegraphics[width=0.5\textwidth]{figs-plots/lifetime-longterm.eps}
      \caption{Creation time distribution of categorized posts over time for WeiboScope dataset. Red boxes present the censored posts and blue boxes the uncensored ones.}
      \label{fig:time-weiboscope}
\end{figure}

\mct{I was expecting to see a plot showing how the rate of censorship changes over creation time.}


\subsection{Caveats}
When interpreting our results, one should keep in mind that our results are based on two datasets that track different user populations of Weibo. The Zhu2012 dataset is based on a specific core set of sensitive users which might not represent the Weibo's general population. On the other hand, since WeiboScope tracks a larger number of users, its data might be more representative of the general population of Weibo.


%Another caveat about our methodology is that we don't take into account whether an image in a specific category is in favor of China or against it. For example, when we say 54\% of Mao Zedong images are censored, it means that our classifier found 54\% of his images in the censordd category, but we of Xi Xinping might be in favor of China.
